Causal Consistency for Reversible Multiparty Protocols

In programming models with a reversible semantics, computational steps can be undone. This paper addresses the integration of reversible semantics into process languages for communication-centric systems equipped with behavioral types. In prior work, we introduced a monitors-as-memories approach to seamlessly integrate reversible semantics into a process model in which concurrency is governed by session types (a class of behavioral types), covering binary (two-party) protocols with synchronous communication. The applicability and expressiveness of the binary setting, however, is limited. Here we extend our approach, and use it to define reversible semantics for an expressive process model that accounts for multiparty (n-party) protocols, asynchronous communication, decoupled rollbacks, and abstraction passing. As main result, we prove that our reversible semantics for multiparty protocols is causally-consistent. A key technical ingredient in our developments is an alternative reversible semantics with atomic rollbacks, which is conceptually simple and is shown to characterize decoupled rollbacks.

==> intro.tex <==
This paper is about \emph{reversible computation} in the context of  models of concurrency for \emph{communication-centric} software systems, i.e., 
collections of distributed software components whose 
concurrent interactions 
are governed by reciprocal dialogues or \emph{protocols}.

Building upon process calculi techniques, 
these 
models  provide a rigorous footing for %programming languages featuring 
message-passing concurrency; on top of them, many (static) analysis techniques based on \emph{(behavioral) types}  and \emph{contracts} have been put forward  
to enforce key safety and liveness properties~\cite{DBLP:journals/csur/HuttelLVCCDMPRT16}. Reversibility is an appealing notion in concurrency at large~\cite{DBLP:journals/eatcs/Lanese14}, but especially so in communication-centric scenarios: it may elegantly abstract fault-tolerant communicating systems that react to  unforeseen circumstances (say, local failures) by ``undoing'' computation steps so as to reach a consistent previous state.
%As such, reversibility is related to process constructs such as exceptions, compensations,  and transactions (see, e.g.,~\cite{DBLP:conf/concur/DanosK05,DBLP:conf/concur/CarboneHY08,DBLP:conf/concur/VriesKH10,DBLP:books/sp/sensoria2011/FerreiraLRVZ11}).
%\jp{I would try to mention/cite connections between `declarative programming' and reversibility here.}

In communication-centric software systems, protocols
specify the intended communication structures among interacting components. 
We focus on process calculi equipped with behavioral types, which use those protocols as types to enforce communication correctness. The interest is in different flavors of \emph{protocol conformance}, i.e., properties that ensure that each component respects its ascribed protocol. The integration of reversibility in models of communication-centric systems has been addressed from various angles (cf. \cite{DBLP:journals/jlp/TiezziY15,DBLP:conf/rc/TiezziY16,DBLP:journals/fac/BarbaneraDd16,DBLP:journals/corr/MezzinaP16}). Focusing on \emph{session types}~\cite{honda.vasconcelos.kubo:language-primitives,HYC08} (a well established class of behavioral types), Tiezzi and Yoshida~\cite{DBLP:journals/jlp/TiezziY15} were the first to integrate reversibility into a session $\pi$-calculus, following the seminal approach of Danos and Krivine~\cite{DanosK04}; in~\cite{DBLP:journals/jlp/TiezziY15}, however, session types are not used in the definition of reversible communicating systems, nor play a role in establishing their properties. 

Triggered by this observation,  our prior work~\cite{DBLP:journals/corr/MezzinaP16,MezzinaP17} develops a \emph{monitors-as-memories} approach. The idea is to use \emph{monitors} (run-time entities that enact protocol actions) as the \emph{memories} needed to record  and   undo communication steps. 
There is a monitor for each protocol participant; 
the monitor includes a session type that describes the intended protocol. 
We use a  \emph{cursor}  to ``mark'' the current protocol state in the type; the cursor can move to the future (enacting protocol actions) but also to the past (reversing protocol actions). The result is a streamlined process framework in which the key properties of a reversible semantics can be established with simple proofs,
because session types narrow down the spectrum of possible process behaviors, allowing only those forward and backward actions that correspond to the declared protocols.
The most significant of such properties is 
\emph{causal consistency}~\cite{DanosK04},   considered as the ``right''  criterion for reversing concurrent processes~\cite{DBLP:journals/eatcs/Lanese14}. 
Intuitively, causal consistency ensures that reversible steps lead to system states that could been have reached by performing forward steps only. That is, causally consistent reversibility does not lead to extraneous states, not reachable through ordinary computations.

The  framework in~\cite{DBLP:journals/corr/MezzinaP16,MezzinaP17}, however,  accounts only for reversible  $\pi$-calculus processes implementing \emph{binary sessions}, i.e., protocols between exactly two partners. Also, it considers \emph{synchronous communication} instead of the more general (and practical) \emph{asynchronous (queue-based) communication}. 
Hence, our prior work %does not cover the 
%\emph{multiparty asynchronous sessions}~\cite{HYC08} that may describe protocols between two or more parties. Thus,~\cite{DBLP:journals/corr/MezzinaP16} 
rules out an important class of real-life protocols, namely the 
\emph{choreographies} that  describe  interaction scenarios among multiple parties without a single point of control. 
In \emph{multiparty session types}~\cite{HYC08}, these choreographies are represented by a \emph{global type} that can be projected as \emph{local types} to obtain each participant's contribution to the entire interaction. 
Moving from binary to multiparty sessions is a significant jump in expressiveness;
\added{in fact, global types offer a convenient declarative description of the entire communication scenario.}
However, the multiparty case also  
entails added challenges, as  two levels of abstraction, global and local, should be considered for (reversible) protocols and their   implementations. Hence, it is far from obvious that our monitors-as-memories approach to reversibility and  causal consistency extend to the multiparty case.
%\footnote{Indeed, the principled transfer of  techniques from binary to multiparty settings has been clarified only recently~\cite{DBLP:conf/forte/CairesP16}.}

%\paragraph{Contributions} 
%The \emph{main contribution} of this paper is the extension of the monitors-as-memories approach to multiparty asynchronous sessions. 
This paper makes the following contributions:

\begin{itemize}%[1.]
\item We introduce a process model for reversible, multiparty sessions with asynchrony (as in~\cite{DBLP:journals/mscs/KouzapasYHH16}), process passing~\cite{SangiorgiD:expmpa,KPY2016} and decoupled rollbacks (\S\,\ref{s:calculus}). 
We define forward and backward semantics for multiparty processes by extending the monitors-as-memories approach to both
global types and their implementations. 

\item  We prove that reversibility in our model is causally consistent (Theorem~\ref{t:causal}). The proof is challenging as we must appeal to an alternative reversible semantics with 
\emph{atomic rollbacks}, which we show to coincide with the decoupled rollbacks (Theorem~\ref{t:bf}). 

\item We formally connect reversibility at the (declarative) level of global types
and that at the (operational) level of processes monitored by local types with cursors (Theorem~\ref{t:corrgc}).
\end{itemize}

%, so we improve over our prior work already at the level of processes. 
\noindent 
We stress that asynchrony, process passing, and decoupled rollbacks are not considered in prior works~\cite{DBLP:conf/rc/TiezziY16,DBLP:journals/corr/Dezani-Ciancaglini16a,DBLP:journals/corr/MezzinaP16,MezzinaP17}.
Asynchrony  and decoupled rollbacks are delicate issues in a reversible multiparty setting---we do not know of other asynchronous calculi with reversible semantics, nor featuring the same combination of constructs. 
The formal connection between global and local levels of abstraction (Theorem~\ref{t:corrgc}) is also unique to our multiparty setting.

\paragraph{Organization}
This paper is organized as follows. In \S\,\ref{s:calculus}, we introduce our process model of reversible choreographies. 
We illustrate the model by means of an example in \S\,\ref{s:examp}.
In \S\,\ref{s:results} we establish causal consistency by relating decoupled and atomic semantics, and connect reversibility at global and local levels. 
\S\,\ref{s:ext} discusses extensions to our framework, while 
\S\,\ref{s:rw} contrasts with related works.
\S\,\ref{s:conc} collects some concluding remarks and directions for future work. 
%\emph{For the sake of space, some definitions/proofs are relegated to the appendix.}
\emph{The appendix contains additional material.}
Omitted definitions/proofs can be found in an online technical report~\cite{MezzinaP17arxiv}.


==> macros.tex <==
% !TEX root = revchor.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Contents
% --------

% 1.  Formating
% 2.  Maths - Theorems
% 3.  The pi Calculus
% 4.  Session Syntax
% 5.  Subject Reduction
% 6.  Global Session Types
% 7.  Global Session Types Equivalence
% 8.  Projection
% 9.  Local Session Types
% 10. Behavioural Theory
% 11. Typed Transitions - Reductions
% 12. Typed Relations
% 13. Confluence Determinacy
% 14. Mapping
% 15. pi Constructs
% 16. LN Transform
% 17. General Types Processes Names Sessions ETC
% 18. newtheorem - newenvironment
% 19. Misc
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       FORMATING
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Symbols
\newcommand{\semicolon}{:}
%\newcommand{\colon}{;}
\newcommand{\lrangle}[1]{\langle #1 \rangle}
\newcommand{\blrangle}[1]{\big\langle #1 \big\rangle}

%Tags
\newcommand{\parenthtext}[1]{(\textrm{\small #1})}
\newcommand{\brtext}[1]{[\textrm{\small #1}]}
\newcommand{\textinmath}[1]{\textrm{#1}}
\newcommand{\srule}[1]{\parenthtext{#1}}
\newcommand{\strule}[1]{\textrm{#1}}
\newcommand{\stypes}[1]{{\footnotesize \parenthtext{#1}}}
\newcommand{\ltsrule}[1]{{\footnotesize \lrangle{\textrm{#1}}}}
\newcommand{\eltsrule}[1]{{\footnotesize [\textrm{#1}]}}
\newcommand{\trule}[1]{{\footnotesize\brtext{#1}}}
\newcommand{\orule}[1]{{\scriptsize{\brtext{#1}}}}
\newcommand{\mrule}[1]{{\footnotesize{\parenthtext{#1}}}}

\newcommand{\iftag}{{\textrm{if }}}

% General
\newcommand{\noi}{\noindent}
\newcommand{\Hline}{\rule{\linewidth}{.5pt}}
\newcommand{\Hlinefig}{\rule{\linewidth}{.5pt}\vspace{-4mm}}
\newcommand{\myparagraph}[1]{\noindent{\textbf{#1}\ }}
\newcommand{\jparagraph}[1]{\paragraph{\textbf{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                       MATHS - THEOREMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\newtheorem{notation}[definition]{Notation}

% BNF form
\newcommand{\bnfis}{\;\;::=\;\;}
\newcommand{\bnfbar}{\;\;\;|\;\;\;}
\newcommand{\sbnfbar}{\;|\;}

% Proof
\newcommand{\Case}[1]{\noi {\bf Case: }#1\\}
\newcommand{\proofend}{\qed}
%\newcommand{\proofend}{}
\newcommand{\Proof}{\noi {\bf Proof: }}

% Logic
\newcommand{\LogAnd}{\texttt{ and }}
\newcommand{\LogOr}{\texttt{ or }}

% Induction

\newcommand{\basic}{\noi {\bf Basic Step:}\\}
\newcommand{\inductive}{\noi {\bf Inductive Hypothesis:}\\}
\newcommand{\induction}{\noi {\bf Induction Step:}\\}

% Tree

\newcommand{\tree}[2]{
\ensuremath{\displaystyle
		\frac
		{
			%%\raisebox{0.0mm}{$\displaystyle{#1}$}
			#1
			%\vspace{0mm}
		}{
			%\vspace{2mm}
			#2
			%\raisebox{-0.4mm}{$\displaystyle{#2}$}
		}
	}
}


%\newcommand{\tree}[2]{
%\begin{prooftree}
%	#1
%	\justifies
%	#2
%\end{prooftree}
%}

\newcommand{\treeusing}[3]{
\begin{prooftree}
	#1
	\justifies
	#2
	\using
	#3
\end{prooftree}}

% Vectors
\newcommand{\vect}[1]{\tilde{#1}}
\newcommand{\mytilde}[1]{\widetilde{#1}}

% Functions - Set theory
\newcommand{\set}[1]{\{#1\}}
\newcommand{\es}{\emptyset}
\newcommand{\maxset}[1]{\max(#1)}
\newcommand{\setbar}{\ \ |\ \ }
\newcommand{\tuple}[2]{(#1, #2)}
\newcommand{\suchthat}{\cdot}
\newcommand{\powerset}[1]{\mathcal{P}(#1)}
\newcommand{\product}{\times}

\newcommand{\eval}{\downarrow}

\newcommand{\setsubtr}[2]{#1 \backslash #2}

\newcommand{\func}[2]{#1(#2)}
\newcommand{\dom}[1]{\mathtt{dom}(#1)}
\newcommand{\codom}[1]{\mathtt{codom}(#1)}

\newcommand{\funcbr}[2]{#1\lrangle{#2}}

\newcommand{\entails}{\text{implies}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                        pi - CALCULUS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Free-Bound notation
\newcommand{\freev}[1]{\lrangle{#1}}
\newcommand{\boundv}[1]{(#1)}

% General pi calculus Syntax
\newcommand{\send}[1]{\overline{#1}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\receive}[1]{#1.}
\newcommand{\inact}{\mathbf{0}}
\newcommand{\If}{\sessionfont{if}\ }
\newcommand{\Then}{\sessionfont{then}\ }
\newcommand{\Else}{\sessionfont{else}\ }
\newcommand{\ifthen}[2]{\If #1\ \Then #2\ }
\newcommand{\ifthenelse}[3]{\ifthen{#1}{#2} \Else #3}
\newcommand{\Par}{\;|\;}
\newcommand{\news}[1]{(\nu\, #1)}
\newcommand{\newsp}[2]{(\nu\, #1)(#2)}
\newcommand{\varp}[1]{#1}
%\newcommand{\rvar}[1]{\mathcal{#1}}
\newcommand{\rvar}[1]{#1}
%\newcommand{\rec}[2]{\mu #1. #2}
\newcommand{\recp}[2]{\mu \rvar{#1}. #2}

\newcommand{\Def}{\sessionfont{def}\ }

\newcommand{\defeq}{\stackrel{\Def}{=}}

\newcommand{\repl}{\ast\,}
\newcommand{\parcomp}[2]{\prod_{#1}{#2}}

% Free-Bound-Names sets
\newcommand{\bn}[1]{\mathtt{bn}(#1)}
\newcommand{\fn}[1]{\mathtt{fn}(#1)}
\newcommand{\sn}[1]{\mathtt{sn}(#1)}
\newcommand{\ofn}[1]{\mathsf{ofn}(#1)}
\newcommand{\fv}[1]{\mathtt{fv}(#1)}
\newcommand{\bv}[1]{\mathtt{bv}(#1)}
\newcommand{\fs}[1]{\mathtt{fs}(#1)}
\newcommand{\fpv}[1]{\mathtt{fpv}(#1)}
\newcommand{\nam}[1]{\mathtt{n}(#1)}

%Subject - Object
\newcommand{\subj}[1]{\mathtt{subj}(#1)}
\newcommand{\obj}[1]{\mathtt{obj}(#1)}

% Relations
\newcommand{\relfont}[1]{\mathcal{#1}}
\newcommand{\rel}[3]{#1\ \relfont{#2}\ #3}

\newcommand{\scong}{\equiv}
\newcommand{\acong}{\scong_{\alpha}}
\newcommand{\wb}{\approx}
\newcommand{\fwb}{\approx^\mathtt{C}}
\newcommand{\hwb}{\approx^\mathtt{H}}
\newcommand{\swb}{\approx^{s}}
\newcommand{\wbc}{\approx}
\newcommand{\WB}{\approx}

\newcommand{\red}{\longrightarrow}
\newcommand{\Red}{\rightarrow\!\!\!\!\!\rightarrow}
\newcommand{\Redleft}{\leftarrow\!\!\!\!\!\leftarrow}

%\newcommand{\subst}[2]{\set{#1/#2 }}
\def\subst#1#2{\{\raisebox{.5ex}{\small$#1$}\! / \mbox{\small$#2$}\}}

% Context
\newcommand{\hole}{-}
\newcommand{\context}[2]{#1[#2]}
\newcommand{\Ccontext}[1]{\C[#1]}

% Expression Context
\newcommand{\Econtext}[1]{\E[#1]}

% Barbs
\newcommand{\barb}[1]{\downharpoonright_{#1}}
\newcommand{\Barb}[1]{\Downarrow_{#1}}
\newcommand{\nbarb}[1]{\not\downarrow_{#1}}
\newcommand{\nBarb}[1]{\not\Downarrow_{#1}}

% General
%\newcommand{\ESP}{\ensuremath{\mathbf{ESP}}}
\newcommand{\ESP}{\text{ESP}}
\newcommand{\ESPsel}{\ESP^+}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                        SESSION SYNTAX
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Session font
\newcommand{\sessionfont}[1]{\mathtt{#1}}
\newcommand{\vart}[1]{\mathsf{#1}}

% General Session symbols
\newcommand{\ssep}{;}
\newcommand{\shsep}{.}
\newcommand{\outses}{!}
\newcommand{\inpses}{?}
\newcommand{\selses}{\triangleleft}
\newcommand{\brases}{\triangleright}
\newcommand{\dual}[1]{\overline{#1}}
\newcommand{\cat}{\cdot}

\newcommand{\allstypes}{\mathcal{S}}

% Binary Session Syntax


\newcommand{\bacc}[2]{#1 \boundv{#2} \shsep}
\newcommand{\breq}[2]{\send{#1} \freev{#2} \shsep}
\newcommand{\bareq}[2]{\send{#1} \freev{#2}}

\newcommand{\breqt}[3]{\send{#1} \boundv{#2:#3} \shsep}
\newcommand{\bacct}[3]{#1 \boundv{#2:#3} \shsep}

\newcommand{\bout}[2]{#1 \outses \freev{#2} \shsep}
\newcommand{\bbout}[2]{#1 \outses \blrangle{#2} \shsep}
\newcommand{\binp}[2]{#1 \inpses \boundv{#2} \shsep}
\newcommand{\bselold}[2]{#1 \selses #2 \shsep}
\newcommand{\bsel}[2]{#1 \selses \set{#2}}

%\newcommand{\bout}[2]{#1 \outses \freev{#2} \ssep}
%\newcommand{\bbout}[2]{#1 \outses \blrangle{#2} \ssep}
%\newcommand{\binp}[2]{#1 \inpses \boundv{#2} \ssep}
%\newcommand{\bsel}[2]{#1 \selses #2 \ssep}
\newcommand{\bbra}[2]{#1 \brases \set{#2}}
\newcommand{\bbras}[2]{#1 \brases #2}
\newcommand{\bbraP}[1]{#1 \brases \lPi}

% Multiparty Session syntax

\newcommand{\role}[1]{[#1]}

\newcommand{\srole}[2]{#1\role{#2}}
\newcommand{\sqrole}[2]{#1^{[]}\role{#2}}

\newcommand{\fromto}[2]{\role{#1} \role{#2}}
\newcommand{\sfromto}[3]{#1\fromto{#2}{#3}}

\newcommand{\sout}[3]{\srole{#1}{#2} \outses \freev{#3} \ssep}
\newcommand{\sinp}[3]{\srole{#1}{#2} \inpses \boundv{#3} \ssep}
\newcommand{\sdel}[4]{\srole{#1}{#2} \outses \freev{\srole{#3}{#4}} \ssep}
\newcommand{\ssel}[3]{\srole{#1}{#2} \selses #3 \ssep}
\newcommand{\sbra}[3]{\srole{#1}{#2} \brases \set{#3}}
\newcommand{\sbras}[3]{\srole{#1}{#2} \brases #3}
\newcommand{\sbraP}[2]{\srole{#1}{#2} \brases \lPi}

\newcommand{\acc}[3]{#1 \role{#2} \boundv{#3} \shsep}
\newcommand{\req}[3]{\send{#1} \role{#2} \boundv{#3} \shsep}
\newcommand{\areq}[3]{\send{#1} \role{#2} \freev{#3}}

\newcommand{\out}[4]{\sfromto{#1}{#2}{#3} \outses \freev{#4} \ssep}
\newcommand{\inp}[4]{\sfromto{#1}{#2}{#3} \inpses \boundv{#4} \ssep}
\newcommand{\del}[5]{\sfromto{#1}{#2}{#3} \outses \freev{\srole{#4}{#5}} \ssep}
\newcommand{\sel}[4]{\sfromto{#1}{#2}{#3} \selses #4 \ssep}
\newcommand{\bra}[4]{\sfromto{#1}{#2}{#3} \brases \set{#4}}
\newcommand{\bras}[4]{\sfromto{#1}{#2}{#3} \brases #4}
\newcommand{\braP}[3]{\sfromto{#1}{#2}{#3} \brases \lPi}

% Arrive construct
\newcommand{\arrivetext}{\mathtt{arrive}}
\newcommand{\arrive}[1]{\arrivetext\ #1}
\newcommand{\arrivem}[2]{\arrivetext\ #1\ #2}

% Typecase construct
\newcommand{\typecasetext}{\mathtt{typecase}}
\newcommand{\oftext}{\mathtt{of}}
\newcommand{\typecase}[2]{\typecasetext\ #1\ \oftext\ \set{#2}}

% IO symbols
\newcommand{\inputsym}{\mathtt{i}}
\newcommand{\outputsym}{\mathtt{o}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                      SUBJECT REDUCTION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% typing reduction
\newcommand{\typingred}{\red}
\newcommand{\typingRed}{\Red}

\newcommand{\wellconf}[1]{\mathtt{wc}(#1)}
\newcommand{\cohses}[2]{\mathtt{co}(#1(#2))}
\newcommand{\coherent}[1]{\mathtt{co}(#1)}
\newcommand{\fcoherent}[1]{\mathtt{fco}(#1)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                      SESSION ENDPOINTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Asynchronous syntax
%\newcommand{\mareq}[4]{\newsp{\srole{#2}{#3}, \dots, \srole{#2}{#4}}{\send{#1}[#3] \freev{#2} \Par \dots \Par \send{#1}[#4]\freev{#2}}}

%\newcommand{\areqs}[3]{\send{#1}[\set{#2}] \freev{#3}}

% Queues
\newcommand{\emp}{\epsilon}
\newcommand{\squeue}[3]{\srole{#1}{#2}:#3}
\newcommand{\srqueue}[4]{\srole{#1}{#2}[\inputsym: #3, \outputsym: #4]}
\newcommand{\srqueuei}[3]{\srole{#1}{#2}[\inputsym: #3]}
\newcommand{\srqueueo}[3]{\srole{#1}{#2}[\outputsym: #3]}
\newcommand{\srqueueio}[4]{\srole{#1}{#2}[\inputsym: #3, \outputsym: #4]}
\newcommand{\sgqueue}[2]{\srole{#1}:#2}

% Shared Names Queues
\newcommand{\shqueue}[2]{#1[#2]}
%\newcommand{\shqueuet}[3]{#1[#2, #3]}

% IO Queues
\newcommand{\squeueio}[3]{#1[\inputsym: #2, \outputsym: #3]}
\newcommand{\squeuei}[2]{#1[\inputsym: #2]}
\newcommand{\squeueo}[2]{#1[\outputsym: #2]}

\newcommand{\squeuetio}[4]{#1[#2, \inputsym: #3, \outputsym: #4]}
\newcommand{\squeueto}[3]{#1[#2, \outputsym: #3]}
\newcommand{\squeueti}[3]{#1[#2, \inputsym: #3]}
\newcommand{\squeuet}[2]{#1[#2]}

% Queue Values

\newcommand{\queuev}[2]{\role{#1}(#2)}
\newcommand{\queuel}[2]{\role{#1} #2}
\newcommand{\queues}[3]{\role{#1}(\srole{#2}{#3})}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                        GLOBAL SESSION TYPES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\impl}[2]{\{\!\{#1\}\!\}_{\mathcal{#2}}}
\newcommand{\impll}[2]{\{\!\{#1\}\!\}_{\mathcal{#2}}^\fw}

\newcommand{\gtfont}[1]{\mathtt{#1}}
\newcommand{\gsep}{.}

\newcommand{\globaltype}[1]{\lrangle{#1}}
\newcommand{\parties}[1]{\mathtt{\pa}(#1)}
\newcommand{\roles}[1]{\mathtt{roles}(#1)}

\newcommand{\fromtogt}[2]{#1 \rightarrow #2 \semicolon}

\newcommand{\valuegt}[3]{\fromtogt{#1}{#2} \lrangle{#3} \gsep}
\newcommand{\selgt}[3]{\fromtogt{#1}{#2} \set{#3}}
\newcommand{\selgtG}[2]{\fromtogt{#1}{#2} \lGi}
\newcommand{\recgt}[2]{\mu \vart{#1}. #2}
\newcommand{\vargt}[1]{\vart{#1}}
\newcommand{\inactgt}{\gtfont{end}}

\newcommand{\swap}{\ensuremath{\approx_{\mathtt{sw}}}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                              GLOBAL SESSION TYPES EQUIVALENCE
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\projset}[1]{\mathtt{proj}(#1)}
\newcommand{\aprojset}[1]{\mathtt{aproj}\ #1 }
\newcommand{\gcong}{\equiv}
\newcommand{\govcong}{\cong_g}
\newcommand{\gperm}{\simeq}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                        PROJECTION
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\projsymb}{\lceil}
\newcommand{\proj}[2]{#1 \projsymb #2}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                        LOCAL SESSION TYPES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tfont}[1]{\mathtt{#1}}
\newcommand{\tsep}{;}

\newcommand{\chtype}[1]{\lrangle{#1}}
\newcommand{\chtypei}[1]{\inputsym \lrangle{#1}}
\newcommand{\chtypeo}[1]{\outputsym \lrangle{#1}}
\newcommand{\chtypeio}[1]{\inputsym \outputsym \lrangle{#1}}

\newcommand{\outtype}{\outses}
\newcommand{\inptype}{\inpses}
\newcommand{\seltype}{\selses}
\newcommand{\bratype}{\brases}

\newcommand{\trec}[2]{\mu\vart{#1}.#2}
\newcommand{\tvar}[1]{\vart{#1}}
%\newcommand{\settype}[1]{\set{#1}}
\newcommand{\tset}[1]{\set{#1}}
\newcommand{\tinact}{\tfont{end}}

%\newcommand{\sminus}[1]{#1^-}
\newcommand{\sminus}[1]{#1^{\text{--}}}

\newcommand{\subt}{\leq}
\newcommand{\supt}{\geq}

% Multiparty Local Session Types
\newcommand{\tout}[2]{\role{#1} \outtype \lrangle{#2} \tsep}
\newcommand{\tinp}[2]{\role{#1} \inptype (#2) \tsep}
\newcommand{\tsel}[2]{\role{#1} \seltype \set{#2}}
\newcommand{\tsels}[2]{\role{#1} \seltype #2}
\newcommand{\tselT}[1]{\role{#1} \seltype \lTi}
\newcommand{\tbra}[2]{\role{#1} \bratype \set{#2}}
\newcommand{\tbras}[2]{\role{#1} \bratype #2}
\newcommand{\tbraT}[1]{\role{#1} \bratype \lTi}

% Binary Session Types
\newcommand{\btout}[1]{\outtype \lrangle{#1} \tsep}
\newcommand{\bbtout}[1]{\outtype \big\langle{#1}\big\rangle \tsep}
\newcommand{\btinp}[1]{\inptype (#1) \tsep}
\newcommand{\bbtinp}[1]{\inptype \big({#1}\big) \tsep}
\newcommand{\btsel}[1]{\oplus \set{#1}}
\newcommand{\btselS}{\oplus \lSi}
\newcommand{\btbra}[1]{\& \set{#1}}
\newcommand{\btbraS}{\& \lSi}

% Queue Typing

\newcommand{\mtout}[2]{\role{#1} \outtype \lrangle{#2}}
\newcommand{\mtinp}[2]{\role{#1} \inptype (#2)}
\newcommand{\mtsel}[2]{\role{#1} \seltype #2}
\newcommand{\mtbra}[2]{\role{#1} \bratype #2}


% Binary Queue Typing

\newcommand{\bmtout}[1]{\outtype \lrangle{#1}}
\newcommand{\bmtinp}[1]{\inptype (#1)}
\newcommand{\bmtsel}[1]{\seltype #1}
\newcommand{\bmtbra}[1]{\bratype #1}

% Message concatanation
\newcommand{\mcat}{\;*\;}
\newcommand{\icat}{\;\circ\;}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                        TYPED PROCESSES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Ga}{\Gamma}
\newcommand{\De}{\Delta}
\newcommand{\proves}{\vdash}
\newcommand{\hastype}{\triangleright}

\newcommand{\Decat}[1]{\De \cat #1}
\newcommand{\Gacat}[1]{\Ga \cat #1}

\newcommand{\tcat}{\circ}

\newcommand{\typed}[1]{#1:}
\newcommand{\typedrole}[2]{\typed{\srole{#1}{#2}}}
%\newcommand{\typedqrole}[2]{\typed{\srole{#1^{[]}}{#2}}}

\newcommand{\typedprocess}[3]{#1 \proves #2 \hastype #3}

\newcommand{\Eproves}[3]{#1 \proves \typed{#2} #3}
\newcommand{\Gproves}[2]{\Eproves{\Ga}{#1}{#2}}

\newcommand{\tprocess}[3]{#1 \proves #2 \hastype #3}
\newcommand{\Gtprocess}[2]{\tprocess{\Ga}{#1}{#2}}
\newcommand{\Gptprocess}[2]{\tprocess{\Ga'}{#1}{#2}}

\newcommand{\noGtprocess}[2]{#1 \hastype #2}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                    MULTIPARTY TYPED THEORY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\globalenv}[1]{\set{#1}}
%\newcommand{\globalenvI}{\set{\typed{s_i} \G_i}_{i \in I}}
\newcommand{\globalenvI}{E}
\newcommand{\globalenvJ}{\set{\typed{s_j} \G_j}_{j \in J}}

\newcommand{\Gltprocess}[4]{\tprocess{#1}{#2}{#3, #4}}

\newcommand{\geI}{\globalenvI}
\newcommand{\geJ}{\globalenvJ}

\newcommand{\Stprocess}[3]{\tprocess{\geI, #1}{#2}{#3}}
\newcommand{\SGtprocess}[2]{\Gtprocess{#1}{#2, \globalenvI}}
\newcommand{\SJGtprocess}[2]{\globalenvJ, \Gtprocess{#1}{#2}}

\newcommand{\Observer}[2]{\mathsf{Observer}(#1, #2)}
\newcommand{\ObserverG}[1]{\mathsf{Observer}(\globalenvI, #1)}

\newcommand{\Obs}{\ensuremath{\mathsf{Obs}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                        BEHAVIOURAL THEORY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\fromtolts}[2]{\fromto{#1}{#2}}

\newcommand{\outlts}{\outses}
\newcommand{\inplts}{\inpses}
\newcommand{\sellts}{\oplus}
\newcommand{\bralts}{\&}

% Multiparty Labels
\newcommand{\actreq}[3]{\send{#1} \role{#2} \boundv{#3}}
%\newcommand{\actbreq}[3]{\send{#1} \role{#2} \boundv{#3}}

\newcommand{\actreqs}[3]{\send{#1} \role{\set{#2}} \boundv{#3}}
%\newcommand{\actbreqs}[3]{\send{#1} \role{\set{#2}} \boundv{#3}}

\newcommand{\actacc}[3]{#1 \role{#2} \boundv{#3}}
\newcommand{\actaccs}[3]{#1 \role{\set{#2}} \boundv{#3}}

\newcommand{\actout}[4]{#1 \fromtolts{#2}{#3} \outlts \freev{#4}}
\newcommand{\actqout}[4]{#1^{[]} \fromtolts{#2}{#3} \outlts \freev{#4}}
\newcommand{\actbout}[4]{#1 \fromtolts{#2}{#3} \outlts \boundv{#4}}

\newcommand{\actdel}[5]{#1 \fromtolts{#2}{#3} \outlts \freev{\srole{#4}{#5}}}
\newcommand{\actbdel}[5]{#1 \fromtolts{#2}{#3} \outlts \boundv{\srole{#4}{#5}}}
\newcommand{\actqdel}[5]{#1^{[]} \fromtolts{#2}{#3} \outlts \boundv{\srole{#4}{#5}}}

\newcommand{\actinp}[4]{#1 \fromtolts{#2}{#3} \inplts \freev{#4}}
\newcommand{\actqinp}[4]{#1^{[]} \fromtolts{#2}{#3} \inplts \freev{#4}}

\newcommand{\actsel}[4]{#1 \fromtolts{#2}{#3} \sellts #4}
\newcommand{\actqsel}[4]{#1^{[]} \fromtolts{#2}{#3} \sellts #4}

\newcommand{\actbra}[4]{#1 \fromtolts{#2}{#3} \bralts #4}
\newcommand{\actqbra}[4]{#1^{[]} \fromtolts{#2}{#3} \bralts #4}

\newcommand{\actval}[4]{#1: #2 \rightarrow #3:#4}
\newcommand{\actgsel}[4]{#1: #2 \rightarrow #3:#4}

% Binary Labels
\newcommand{\bactreq}[2]{\send{#1} \freev{#2}}
\newcommand{\bactbreq}[2]{\send{#1} \boundv{#2}}
\newcommand{\bactacc}[2]{#1 \freev{#2}}

\newcommand{\bactout}[2]{#1 \outlts \freev{#2}}
\newcommand{\bactbout}[2]{#1\outlts \boundv{#2}}
\newcommand{\bactinp}[2]{#1 \inplts \freev{#2}}
\newcommand{\bactsel}[2]{#1 \sellts #2}
\newcommand{\bactbra}[2]{#1 \bralts #2}

% Labelled transition relations
\newcommand{\by}[1]{\stackrel{#1}{\longrightarrow}}
\newcommand{\By}[1]{\stackrel{#1}{\Longrightarrow}}

\newcommand{\hby}[1]{\stackrel{#1}{\longmapsto}}
\newcommand{\Hby}[1]{\stackrel{#1}{\Longmapsto}}


% Session barbs
\newcommand{\barbreq}[1]{\barb{#1}}
%\newcommand{\barbacc}[2]{\barb{#1\role{\set{#2}}}}
\newcommand{\barbout}[3]{\barb{\sfromto{#1}{#2}{#3}}}
%\newcommand{\barbinp}[3]{\barb{#1\fromto{#2}{#3}\inpses}}

\newcommand{\Barbreq}[2]{\Barb{\send{#1}\role{#2}}}
%\newcommand{\Barbacc}[2]{\Barb{#1\role{\set{#2}}}}
%\newcommand{\Barbout}[3]{\Barb{\sfromto{#1}{#2}{#3}\outses}}
\newcommand{\Barbout}[3]{\Barb{\sfromto{#1}{#2}{#3}}}
%\newcommand{\Barbinp}[3]{\Barb{#1\fromto{#2}{#3}\inpses}}

% Binary Session barbs
\newcommand{\bbarbreq}[1]{\barb{#1}}
%\newcommand{\bbarbacc}[1]{\barb{#1}}
\newcommand{\bbarbout}[1]{\barb{#1}}
%\newcommand{\bbarbinp}[1]{\barb{#1\inpses}}

\newcommand{\bBarbreq}[1]{\Barb{\send{#1}}}
%\newcommand{\bBarbacc}[2]{\Barb{#1}}
\newcommand{\bBarbout}[1]{\Barb{#1\outses}}
%\newcommand{\bBarbinp}[1]{\Barb{#1\inpses}}

\newcommand{\comp}{\asymp}
\newcommand{\coh}{\asymp}
\newcommand{\bistyp}{\rightleftharpoons}

\newcommand{\typingbeh}{\leftrightarrow}

\newcommand{\bufrel}{\succ}

\newcommand{\ordercup}{\bowtie}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                TYPED TRANSITIONS - REDUCTIONS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Environment Transitions
\newcommand{\envtrans}[1]{\by{#1}}
\newcommand{\envTrans}[1]{\by{#1}}
\newcommand{\typedtrans}[1]{\by{#1}}
\newcommand{\typedTrans}[1]{\By{#1}}
\newcommand{\typedred}{\red}
\newcommand{\typedRed}{\Red}

% Typed Environment Transitions - Binary case
\newcommand{\benv}[2]{(#1, #2)}
\newcommand{\bGenv}[1]{\benv{\Ga}{#1}}
\newcommand{\bGDenv}{\envtyp{\Ga}{\De}}

\newcommand{\envby}[5]{\benv{#1}{#2} \envtrans{#3} \benv{#4}{#5}}
\newcommand{\Genvby}[3]{\envby{\Ga}{#1}{#2}{\Ga}{#3}}

% Typed Environment Transitions - Multiparty case

\newcommand{\env}[3]{(#1, #2, #3)}
\newcommand{\Genv}[2]{\env{\globalenvI}{#1}{#2}}
\newcommand{\GGenv}[1]{\env{\globalenvI}{\Ga}{#1}}
\newcommand{\GGDenv}{\env{\globalenvI}{\Ga}{\De}}

% Typed Process Transitions - Binary case

\newcommand{\ftby}[7]{\tprocess{#1}{#2}{#3} \typedtrans{#4} \tprocess{#5}{#6}{#7}}
\newcommand{\ftBy}[7]{\tprocess{#1}{#2}{#3} \typedTrans{#4} \tprocess{#5}{#6}{#7}}

\newcommand{\tpby}[6]{\tprocess{#1}{#2}{#3} \typedtrans{#4} \noGtprocess{#5}{#6}}
\newcommand{\tpBy}[6]{\tprocess{#1}{#2}{#3} \typedTrans{#4} \noGtprocess{#5}{#6}}
\newcommand{\Gtpby}[5]{\Gtprocess{#1}{#2} \typedtrans{#3} \noGtprocess{#4}{#5}}
\newcommand{\GtpBy}[5]{\Gtprocess{#1}{#2} \typedTrans{#3} \noGtprocess{#4}{#5}}

\newcommand{\GGtpby}[5]{\tprocess{\globalenvI, \Ga}{#1}{#2} \typedtrans{#3} \noGtprocess{#4}{#5}}
\newcommand{\GGtpBy}[5]{\tprocess{\globalenvI, \Ga}{#1}{#2} \typedTrans{#3} \noGtprocess{#4}{#5}}

% Typed Reductions - Binary case

\newcommand{\ftpred}[6]{\tprocess{#1}{#2}{#3} \typedred \tprocess{#4}{#5}{#6}}
\newcommand{\ftpRed}[6]{\tprocess{#1}{#2}{#3} \typedRed \tprocess{#4}{#5}{#6}}

\newcommand{\tpred}[5]{\tprocess{#1}{#2}{#3} \typedred \noGtprocess{#4}{#5}}
\newcommand{\tpRed}[5]{\tprocess{#1}{#2}{#3} \typedRed \noGtprocess{#4}{#5}}
\newcommand{\Gtpred}[4]{\Gtprocess{#1}{#2} \typedred \noGtprocess{#3}{#4}}
\newcommand{\GtpRed}[4]{\Gtprocess{#1}{#2} \typedRed \noGtprocess{#3}{#4}}

% Observer Reductions

\newcommand{\obsred}{\red_{obs}}
\newcommand{\obsRed}{\Red_{obs}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                    TYPED RELATIONS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Typed Relations
\newcommand{\fulltrel}[7]{\rel{\typedprocess{#1}{#2}{#3}}{#4}{\typedprocess{#5}{#6}{#7}}}
\newcommand{\treld}[6]{\rel{\typedprocess{#1}{#2}{#3}}{#4}{\noGtypedprocess{#5}{#6}}}
\newcommand{\trel}[5]{\rel{#1 \proves #2}{#3}{\noGtypedprocess{#4}{#5}}}

\newcommand{\tcong}{\cong}
\newcommand{\twb}{\approx}
\newcommand{\govwb}{\approx_g}
\newcommand{\tequiv}{\approx}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                    CONFIGURATION THEORY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\confpair}[2]{(#1, #2)}
\newcommand{\uptoconfpair}[2]{[#1, #2]}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                   CONFLUENCE DETERMINACY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\sesstrans}[1]{\stackrel{#1}{\longrightarrow_{s}}}
\newcommand{\sessTrans}[1]{\stackrel{#1}{\Longrightarrow_{s}}}

\newcommand{\fulltypedsesstrans}[7]{\typedprocess{#1}{#2}{#3} \sesstrans{#4} \typedprocess{#5}{#6}{#7}}
\newcommand{\fulltypedsessTrans}[7]{\typedprocess{#1}{#2}{#3} \sessTrans{#4} \typedprocess{#5}{#6}{#7}}

\newcommand{\typedsesstrans}[6]{\typedprocess{#1}{#2}{#3} \sesstrans{#4} \noGtypedprocess{#5}{#6}}
\newcommand{\typedsessTrans}[6]{\typedprocess{#1}{#2}{#3} \sessTrans{#4} \noGtypedprocess{#5}{#6}}
\newcommand{\Gtypedsesstrans}[5]{\Gtypedprocess{#1}{#2} \sesstrans{#3} \noGtypedprocess{#4}{#5}}
\newcommand{\GtypedsessTrans}[5]{\Gtypedprocess{#1}{#2} \sessTrans{#3} \noGtypedprocess{#4}{#5}}

% Actions
\newcommand{\confact}[2]{#1 \lfloor #2}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                    MAPPING AND ENCODINGS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\map}[1]{[\!\![#1]\!\!]}
\newcommand{\umap}[1]{[\!\![#1]\!\!]^u}
\newcommand{\pmap}[2]{\ensuremath{[\!\![#1]\!\!]^#2}}
\newcommand{\pmapp}[3]{\ensuremath{[\!\![#1]\!\!]^#2_#3}}
\newcommand{\auxmap}[2]{\ensuremath{\{\!\{#1\}\!\}^#2}}
\newcommand{\tauxmap}[2]{\ensuremath{\{\!|#1|\!\}^#2}}
\newcommand{\auxmapp}[3]{\ensuremath{\big\lfloor\!\!\big\lfloor#1\big\rfloor\!\!\big\rfloor^#2_#3}}
\newcommand{\tmap}[2]{\ensuremath{(\!\!\langle#1\rangle\!\!)^{#2}}}
\newcommand{\vtmap}[2]{{\ensuremath{\big\lfloor #1\big\rfloor^{#2}}}}
\newcommand{\mapt}[1]{\ensuremath{(\!\!\langle#1\rangle\!\!)}}
\newcommand{\mapa}[1]{\ensuremath{\{\!\!\{#1\}\!\!\}}}
\newcommand{\namemap}[2]{#1\map{#2}}

\newcommand{\enc}[2]{\big\langle\map{#1}, \mapt{#2}\big\rangle}
\newcommand{\enco}[1]{\big\langle #1\big\rangle}
\newcommand{\encod}[3]{\lrangle{\map{#1}^{#3}, \mapt{#2}^{#3}}}
\newcommand{\fencod}[4]{\lrangle{\map{#1}^{#3}_{#4} \, , \, \mapt{#2}^{#3}}}

\newcommand{\calc}[5]{\lrangle{#1, #2, #3, #4, #5}}
\newcommand{\tyl}[1]{\ensuremath{\mathcal{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                    PI CONSTRUCTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\constrtype}[1]{\mathtt{#1}}


\newcommand{\Let}{\constrtype{let}\ }
\newcommand{\In}{\constrtype{in}\ }
\newcommand{\To}{\constrtype{to}\ }
\newcommand{\new}{\constrtype{new}\ }
\newcommand{\from}{\constrtype{from}\ }
\newcommand{\select}{\constrtype{select}\ }
\newcommand{\register}{\constrtype{register}\ }
\newcommand{\Update}{\constrtype{update}\ }

\newcommand{\selectfrom}[2]{\select #1\ \from #2\ \In}
\newcommand{\registerto}[2]{\register #1\ \To #2\ \In}

\newcommand{\newselector}[1]{\new \constrtype{sel}\ #1\ \In}
\newcommand{\newselectorT}[2]{\new \constrtype{sel}\lrangle{#2}\ #1\ \In}
\newcommand{\selecttype}[1]{\dual{\constrtype{sel}}\lrangle{#1}}
\newcommand{\sselecttype}[1]{\constrtype{sel}\lrangle{#1}}

\newcommand{\update}[3]{\Update(#1, #2, #3)\ \In}

\newcommand{\newenv}[1]{\new \mathtt{env}\ #1\ \In\ }
\newcommand{\Letin}[2]{\Let #1 = #2\ \In}

\newcommand{\selqueue}[2]{#1\lrangle{#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                    DUALITY
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\dualof}{\ \mathsf{dual}\ }


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                        lambda - CALCULUS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\labs}[2]{\lambda #1. #2}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                    HIGHER ORDER SESSION PI
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\pHOp}{\ensuremath{\mathsf{HO}\pi_{\mathsf{p}}}\xspace}
%\newcommand{\pHOpnr}{\ensuremath{\mathsf{HO}\pi^{-\mu}_{\mathsf{p}}}\xspace}
\newcommand{\HOp}{\ensuremath{\mathsf{HO}\pi}\xspace}
%\newcommand{\sessp}{\ensuremath{\mathtt{SE}\pi}\xspace}
\newcommand{\sessp}{\ensuremath{\pi}\xspace}
\newcommand{\haskp}{\ensuremath{\pi^{\lambda}}\xspace}
\newcommand{\pHOp}{\ensuremath{\mathsf{HO}\tilde{\pi}}\xspace}
%\newcommand{\psesp}{\ensuremath{\mathtt{sess}\pi_{\mathsf{p}}}\xspace}
%\newcommand{\psespnr}{\ensuremath{\mathtt{sess}\pi^{-\mu}_{\mathsf{p}}}\xspace}
%\newcommand{\sespnr}{\ensuremath{\mathtt{sess}\pi^{-\mu}}\xspace}
\newcommand{\HO}{\ensuremath{\mathsf{HO}}\xspace}
\newcommand{\HOpp}{\ensuremath{\mathsf{HO\pi^{+}}}\xspace}
\newcommand{\PHOp}{\ensuremath{\mathsf{HO}\,{\widetilde{\pi}}}\xspace}
\newcommand{\PHOpp}{\ensuremath{\mathsf{HO}\,{\widetilde{\pi}}^{\,+}}\xspace}
\newcommand{\PHO}{\ensuremath{\vec{\mathsf{HO}}}\xspace}
\newcommand{\Psessp}{\ensuremath{\vec{\pi}}\xspace}


\newcommand{\CAL}{\ensuremath{\mathsf{C}}\xspace}

%\newcommand{\pol}{\mathsf{p}}


\newcommand{\ST}{\mathsf{ST}}


%\newcommand{\pHO}{\mathsf{pure\ HO}}

%\newcommand{\HOp}{\HO^+}
%\newcommand{\pHOp}{\pHO^+}
%\newcommand{\ppi}{\mathsf{pure\ session\ }\pi}
%\newcommand{\spi}{\mathsf{session\ }\pi}

\newcommand{\Proc}{\ensuremath{\diamond}}


%\newcommand{\appl}[2]{#1\lrangle{#2}}
\newcommand{\appl}[2]{#1\, {#2}}
%\newcommand{\abs}[2]{(#1)#2}
\newcommand{\abs}[2]{\lambda #1.\,#2}

\newcommand{\lollipop}{\multimap}
\newcommand{\sharedop}{\rightarrow}
\newcommand{\logicop}{\multimapdot}

\newcommand{\lhot}[1]{#1\! \lollipop\! \diamond}
\newcommand{\shot}[1]{#1\! \sharedop\! \diamond}
\newcommand{\thunkt}{\ensuremath\{\!\{\diamond\}\!\}}
\newcommand{\thunkp}[1]{\ensuremath\{\!\{#1\}\!\}}
\newcommand{\dummyn}{\ensuremath{\ast}}
\newcommand{\hot}[1]{#1 \logicop \diamond}

%\newcommand{\absmap}[1]{}
\newcommand{\vmap}[1]{|\!|#1|\!|}
\newcommand{\smap}[1]{(\!|\!|#1|\!|\!)^s}
\newcommand{\svmap}[1]{(\!|\!|#1|\!|\!)^{s\rightarrow v}}
\newcommand{\amap}[1]{\mathcal{A}\map{#1}}
\newcommand{\absmap}[2]{\mathcal{A}\map{#1}^{#2}}



%%%%% triggers

\newcommand{\hotrigger}[2]{\binp{#1}{x} \newsp{s}{\appl{x}{s} \Par \bout{\dual{s}}{#2} \inact}}
\newcommand{\fotrigger}[5]{\binp{#1}{#2} \newsp{#3}{\map{#4}^{#3} \Par \bout{\dual{#3}}{#5} \inact}}
%\newcommand{\fotrigger}[2]{\binp{#1}{X} \appl{X}{#2}}

%%%%%% Typed relations

\newcommand{\horel}[6]{#1; #2 \proves #3 #4 #5 \proves #6}
%\newcommand{\horel}[6]{#1; \es; #2 \proves #3 #4 #5 \proves #6}

\newcommand{\mhorel}[7]{
	\begin{array}{rcll}
		#1; \es; #2 &#4& #5 \proves& #3\\
			&#4& #6 & #7
	\end{array}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                    LN TRANSFORM
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Loop}{\mathsf{Loop}}
\newcommand{\CodeBlocks}{\mathsf{CodeBlocks}}

\newcommand{\lnmap}[1]{\namemap{LN}{#1}}
\newcommand{\lnrmap}[1]{\namemap{LNR}{#1}}
\newcommand{\lnblockmap}[1]{\namemap{\mathcal{B}}{#1}}
\newcommand{\lnnonblockmap}[2]{\map{#1, #2}}

\newcommand{\mapenv}[2]{\map{#1}_{#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                        GENERAL TYPES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Values
\newcommand{\true}{\sessionfont{tt}}
\newcommand{\false}{\sessionfont{ff}}

% Typed
\newcommand{\bool}{\sessionfont{bool}}
\newcommand{\nat}{\sessionfont{nat}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                        PROCESSES NAMES SESSIONS ETC
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Processes
\newcommand{\PP}{\ensuremath{P}}
\newcommand{\Q}{\ensuremath{Q}}
\newcommand{\R}{\ensuremath{R}}
\newcommand{\OP}{\ensuremath{\mathsf{O}}}

% Global environments
\newcommand{\En}{\ensuremath{En}}

% Session channels
\newcommand{\s}{\ensuremath{s}}
\newcommand{\ds}{\ensuremath{\dual{s}}}
%\newcommand{\Ms}[2]{\ensuremath{s}\role{#1}\role{#2}}

%Dummy channels
\newcommand{\sd}{\mathtt{sd}}
\newcommand{\shd}{\mathtt{shd}}

% Names
\newcommand{\Ia}{\ensuremath{a}}
\newcommand{\Iu}{\ensuremath{u}}

% Variables, values, expressions
\newcommand{\x}{\ensuremath{x}}
\newcommand{\y}{\ensuremath{y}}
\newcommand{\ks}{\ensuremath{k}}
\newcommand{\cc}{\ensuremath{c}}
\newcommand{\va}{\ensuremath{v}}
%\newcommand{\e}{\ensuremath{e}}
\newcommand{\n}{\ensuremath{n}}

% Process Variables

\newcommand{\X}{\varp{X}}
\newcommand{\Y}{\varp{Y}}

% Roles
\newcommand{\p}{\ensuremath{\mathtt{p}}\xspace}
\newcommand{\pa}{\ensuremath{\mathtt{pa}}}
\newcommand{\q}{\ensuremath{\mathtt{q}}\xspace}
\newcommand{\er}{\ensuremath{\mathtt{r}}}
\newcommand{\A}{\ensuremath{A}}

% Types
%\newcommand{\G}{\ensuremath{G}}
\newcommand{\gG}{\globaltype{\G}}
%\newcommand{\U}{\ensuremath{U}}
\newcommand{\So}{\ensuremath{S}}
\newcommand{\T}{\ensuremath{T}}

% Queue Types
\newcommand{\M}{\ensuremath{M}}
\newcommand{\I}{\ensuremath{M_\inputsym}}
\newcommand{\Om}{\ensuremath{M_\outputsym}}
\newcommand{\Typ}{\ensuremath{\mathsf{T}}}

% Queues values
\newcommand{\h}{\ensuremath{h}}

%barbs
\newcommand{\m}{\ensuremath{\mu}}

% Contexts
%\newcommand{\C}{\ensuremath{{\mathbb{C}}}}
\newcommand{\E}{\ensuremath{E}}

% Congruence completness - Definibility
\newcommand{\TT}{\ensuremath{T}}
\newcommand{\suc}{\textrm{succ}}
\newcommand{\fail}{\textrm{fail}}


% Set selection labels
\newcommand{\lPi}{\set{l_i:\PP_i}_{i \in I}}
\newcommand{\lGi}{\set{l_i:\G_i}_{i \in I}}
\newcommand{\lTi}{\set{l_i:\T_i}_{i \in I}}
\newcommand{\lSi}{\set{l_i:\So_i}_{i \in I}}

% Selector proof

\newcommand{\SEL}{P_\mathit{Sel}}
\newcommand{\DSEL}{P_\mathit{DSel}}
\newcommand{\Sel}{\mathsf{Sel}}
\newcommand{\IfSel}{\mathsf{IfSel}}
\newcommand{\DSel}{\mathsf{DSel}}
\newcommand{\PSel}{\mathsf{PermSel}}
\newcommand{\PIfSel}{\mathsf{PermIfSel}}
\newcommand{\PDSel}{\mathsf{PermDSel}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                        ENVIRONMENTS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newtheorem{fact}{Fact}[section]
\newtheorem{notation}[thm]{Notation}
%\newtheorem{remark}{Remark}

%\newenvironment{notation}{\paragraph{{\bf Notation}}}{}

%\newtheorem{proposition}[fact]{{\bf\em Proposition}}
%\newtheorem{example}[fact]{{\bf\em Example}}
%\newtheorem{lemma}[fact]{{\bf\em Lemma}}
%\newtheorem{corollary}[fact]{{\bf\em Corollary}}
%\newtheorem{definition}[fact]{{\bf\em Definition}}
%\newtheorem{theorem}[fact]{{\bf\em Theorem}}
%\newtheorem{remark}[fact]{{\bf\em Remark}}

\newcommand{\nonhosyntax}[1]{\colorbox{lightgray}{\ensuremath{#1}}}
\newcommand{\nonpisyntax}[1]{\fcolorbox{black}{white}{\ensuremath{#1}}}
\newcommand{\rtsyn}[1]{\fcolorbox{black}{white}{\ensuremath{#1}}}

\newenvironment{mytheorem}{%\vspace{-3pt}
	\begin{theorem}
}{%\vspace{-4pt}
	\end{theorem}
}

\newenvironment{myproposition}{
	\begin{proposition}%\vspace{-3pt}
}{%\vspace{-4pt}
	\end{proposition}
}

\newenvironment{mycorollary}{
	\begin{corollary}%\vspace{-3pt}
}{%\vspace{-4pt}
	\end{corollary}
}

\newenvironment{mylemma}{
	\begin{lemma}%\vspace{-3pt}
}{%\vspace{-4pt}
	\end{lemma}
}


\newenvironment{mydefinition}{%\vspace{-3pt}
	\begin{definition}
}{%\vspace{-3pt}
	\end{definition}
}

%\newenvironment{proof}{
%	{\em Proof.}
%}{}


%\newcommand{\qed}{\ensuremath{\square}}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                        MISC
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\Appendix}[1]{Appendix \ref{#1}}

\newcommand{\dimcom}[1]{{\bf Comment: #1 \\}}

\newcommand{\hintcom}[1]{{\bf Hint: #1 \\}}

\newif\ifny\nyfalse
%\nytrue
\newcommand{\NY}[1]
{\ifny{\color{purple}{#1}}\else{#1}\fi}

\newcommand{\KH}[1]
{\ifny{\color{brown}{#1}}\else{#1}\fi}

\newif\ifdm\dmtrue
%\dmfalse
\newcommand{\dk}[1]
{\ifdm{\color{blue}{#1}}\else{#1}\fi}

\newif\ifrhu\rhutrue
%\rhufalse
\newcommand{\rh}[1]
{\ifdm{\color{red}{#1}}\else{#1}\fi}

\newif\ifjp\jptrue
%\jpfalse
%\newcommand{\jp}[1]
%{\ifjp{\color{red}{#1}}\else{#1}\fi}

\newif\ifjp\jptrue
\jpfalse
\newcommand{\jpc}[1]
{\ifjp{\color{red}{#1}}\else{#1}\fi}


%\newcommand{\newj}[1]{\textcolor{red}{#1}}
\newcommand{\newj}[1]{{#1}}
%\newcommand{\newjb}[1]{\textcolor{blue}{#1}}
\newcommand{\newjb}[1]{{#1}}

\newcommand{\ENCan}[1]{\langle #1 \rangle}
\newcommand{\NI}{\noindent}


\newcommand{\syntaxvspace}{\\[1mm]}

\newcommand{\TO}[2]{#1\to #2}
\newcommand{\GS}[3]{\TO{#1}{#2}\colon \!\ENCan{#3}}

\newcommand{\ASET}[1]{\{#1\}}
\newcommand{\participant}[1]{\mathtt{#1}}
\newcommand{\CODE}[1]{{\tt #1}}

\newcommand{\AT}[2]{#1 \! : \! #2}


\newcommand{\myrm}{}


\newcommand{\secref}[1]{\S\,\ref{#1}}
\newcommand{\defref}[1]{Def.~\ref{#1}}
\newcommand{\notref}[1]{Not.~\ref{#1}}
\newcommand{\defsref}[1]{Defs.~\ref{#1}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\thmref}[1]{Thm.~\ref{#1}}
\newcommand{\thmsref}[1]{Thms.~\ref{#1}}
\newcommand{\exref}[1]{Ex.~\ref{#1}}
\newcommand{\propref}[1]{Prop.~\ref{#1}}
\newcommand{\propsref}[1]{Props.~\ref{#1}}
\newcommand{\appref}[1]{App.~\ref{#1}}
\newcommand{\lemref}[1]{Lem.~\ref{#1}}



\newcommand{\stytra}[6]{\ensuremath{#1; #3 \proves #4 \hby{#2} #5 \proves #6 }}
\newcommand{\stytraarg}[7]{\ensuremath{#1; #3 \proves_{#7} #4 \hby{#2} #5 \proves_{#7} #6 }}
\newcommand{\stytraargi}[8]{\ensuremath{#1; #3 \proves_{#7} #4 \hby{#2}_{#8} #5 \proves_{#7} #6 }}
\newcommand{\wtytra}[6]{\ensuremath{#1; #3 \proves #4 \Hby{#2}  #5 \proves #6}}
\newcommand{\wtytraarg}[7]{\ensuremath{#1; #3 \proves_{#7} #4 \Hby{#2}  #5 \proves_{#7} #6 }}
\newcommand{\wtytraargi}[8]{\ensuremath{#1; #3 \proves_{#7} #4 \Hby{#2}_{#8}  #5 \proves_{#7} #6 }}
\newcommand{\wbb}[6]{\ensuremath{#1; #3 \proves #4 \wb #5 \proves #6 }}
\newcommand{\wbbarg}[7]{\ensuremath{#1; #3 \proves_{#7} #4 \wb_{#7} #5 \proves_{#7} #6 }}

\newcommand{\minussh}{\ensuremath{\mathsf{-sh}}\xspace}

\definecolor{lightgray}{gray}{0.75}

\newcommand\greybox[1]{%
  \vskip\baselineskip%
  \par\noindent\colorbox{lightgray}{%
    \begin{minipage}{\textwidth}#1\end{minipage}%
  }%
  \vskip\baselineskip%
}

%\newcommand{\myparagraph}[1]{\paragraph{\bf #1}}

\newcommand{\mapchar}[2]{\ensuremath{[\!\!(#1)\!\!]^{#2}}}
\newcommand{\omapchar}[1]{\ensuremath{[\!\!(#1)\!\!]_{\mathsf{c}}}}

\newcommand{\trigger}[3]{#1 \leftarrow\!\!\!\!\!\!\!\leftarrow #2:#3 }
%\newcommand{\htrigger}[2]{#1 \Leftarrow #2}
\newcommand{\ftrigger}[3]{#1 \Leftarrow \AT{#2}{#3}}
\newcommand{\htrigger}[2]{#1 \hookleftarrow #2}

\newcommand{\btau}{\tau_{\beta}}
\newcommand{\stau}{\tau_{s}}
\newcommand{\dtau}{\tau_{d}}



%\newcommand{\HOpp}{\ensuremath{\mathsf{HO\pi^{+}}}\xspace}
%\newcommand{\PHOp}{\ensuremath{\mathsf{HO}{\vec{\pi}}}\xspace}
%\newcommand{\PHOpp}{\ensuremath{\mathsf{HO}{\vec{\pi}}^{+}}\xspace}

%%CLAUDIO MACROS%%
\newcommand{\procs}{\mathcal{P}}
\newcommand{\confs}{\mathcal{M}}
\newcommand{\agents}{\mathcal{A}}
%\newcommand{\keyword}[1]{\mathtt{#1}}
\newcommand{\newg}[1]{\keyword{new }\,(#1)}
\newcommand{\cm}[1]{\textcolor{blue}{[CM: #1]}}
\newcommand{\jp}[1]{\textcolor{red}{[JP: #1]}}
\newcommand{\added}[1]{\textcolor{blue}{#1}}
%\newcommand{\added}[1]{#1}fw

%%Reversible%%
\newcommand{\fwcolor}[1]{\textcolor{blue}{#1}}
\newcommand{\bkcolor}[1]{\textcolor{red}{#1}}

\newcommand{\rmark}{\blacklozenge}
\newcommand{\normark}{\lozenge}
\newcommand{\hnormark}{\bkcolor{\circ}}


\newcommand{\key}[2]{#1[#2]}
\newcommand{\np}[2]{#1:#2}
\newcommand{\ep}[2]{#1[#2]}
\newcommand{\mysepp}{\cdot}
\newcommand{\mysep}{\,,\,}
\newcommand{\store}{\sigma}
\newcommand{\queue}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\mytagg}{\spadesuit}
\newcommand{\monig}[4]{\ensuremath{{#1\queue{\textcolor{black}{#2}\mysepp #3\mysepp #4}^{\mytagg}}}}
\newcommand{\moni}[4]{\ensuremath{{#1\queue{\textcolor{black}{#2}\mysepp #3\mysepp #4}}}}
\newcommand{\hmoni}[4]{\ensuremath{{#1\queue{\textcolor{black}{#2}\mysepp #3\mysepp #4}^{\normark}}}}
\newcommand{\monir}[4]{\ensuremath{{#1\queue{\textcolor{black}{#2}\mysepp #3\mysepp #4}^{\bkcolor{\rmark}}}}}
%\newcommand{\moni}[5]{\ensuremath{#1\queue{#2\mysepp #3\mysepp #4\mysepp #5}}}
\newcommand{\mem}[3]{\ensuremath{#1\queue{#2\mysep #3}}}
\newcommand{\past}{\,\textcolor{magenta}{\text{\textbf{\textasciicircum\!\!\textasciicircum}}}}
%\newcommand{\past}{\,\textcolor{magenta}{\ensuremath{ ^\blacktriangle}}\,}
%\newcommand{\past}{\,\textcolor{magenta}{\ensuremath{ ^\curlywedge}}\,}
\newcommand{\typeOut}[2]{#1\outtype \langle #2\rangle}
\newcommand{\typeIn}[2]{#1\inptype ( #2)}

%\newcommand{\coda}[3]{#1:(#2\,:\,#3)}
\newcommand{\coda}[2]{#1:#2}
\newcommand{\history}{\textcolor{magenta}{\mathbf{\star}}}
\newcommand{\codah}[4]{\coda{#1}{(#2\,\history\,#3)\!#4}}
\newcommand{\len}{\mathtt{len}}
\newcommand{\anyv}{m}
\newcommand{\equivq}{\equiv_\mathsf{q}}
%\newcommand{\cons}{::}

\newcommand{\cons}{\circ}
\newcommand{\consh}{\circledwedge}
\newcommand{\valueq}[3]{(#1 \,,\, #2 \,,\,#3)}
\newcommand{\myeval}[2]{#2(#1)}
\newcommand{\ctx}[1]{\mathbb{#1}}
\newcommand{\myctx}[2]{\ctx{#1}[#2]}
\newcommand{\myctxb}[2]{{#1\left[\textcolor{black}{#2}\right]}}
\newcommand{\myctxr}[2]{{#1\left[\textcolor{black}{#2}\right]}}
\newcommand{\freeze}[1]{\left\langle #1 \right\rangle}
\newcommand{\upd}[2]{[#1\mapsto #2]}
\newcommand{\rup}[2]{#1\setminus #2}
\newcommand{\restrict}[1]{\downarrow_{#1}}
\newcommand{\loc}{\ell}	
\newcommand{\myloc}[2]{#1\left\{#2\right\}}	
\newcommand{\lbl}{l}	
%\newcommand{\nil}{\epsilon}

%% example
\newcommand{\epS}{\ep{s}{\mathtt{S}}}
\newcommand{\pS}{\ensuremath{\mathtt{S}}\xspace}
\newcommand{\epA}{\ep{s}{\mathtt{A}}}
\newcommand{\pA}{\ensuremath{\mathtt{A}}\xspace}
\newcommand{\epB}{\ep{s}{\mathtt{B}}}
\newcommand{\pB}{\ensuremath{\mathtt{B}}\xspace}
\newcommand{\epC}{\ep{s}{\mathtt{C}}}
\newcommand{\pC}{\ensuremath{\mathtt{C}}\xspace}
\newcommand{\exBook}{\text{`Logicomix'}}

%% global types
\newcommand{\gend}{\mathtt{end}}
\newcommand{\lend}{\mathsf{end}}
\newcommand{\gpart}[1]{\mathtt{#1}}
\newcommand{\gtact}[5]{\gpart{#1}\to\gpart{#2}:\{#3\langle #4\rangle.#5\}_{i \in I}}
\newcommand{\gtactp}[5]{\gpart{#1}\to\!\past \gpart{#2}:#3\langle #4\rangle.#5}
\newcommand{\gtactpp}[3]{\gpart{#1}\to \gpart{#2}: \past#3}
\newcommand{\gtcho}[4]{\gpart{#1}\to\gpart{#2}:\{#3:#4\}_{i \in I}}
\newcommand{\gtchoi}[5]{\gpart{#1}\to\gpart{#2}:\{#3{:}#4\}_{#5}}
\newcommand{\gtcom}[4]{\gpart{#1}\to\gpart{#2}:\langle #3\rangle.#4}

\newcommand{\lsend}[4]{\gpart{#1}!\{#2\langle #3\rangle.#4\}_{i \in I}}
\newcommand{\lrecv}[4]{\gpart{#1}?\{#2\langle #3\rangle.#4\}_{i \in I}}

%%%% NEW LOCAL TYOES
\newcommand{\ltout}[3]{\gpart{#1}!\langle#2\rangle.#3}
\newcommand{\ltinp}[3]{\gpart{#1}?\langle#2\rangle.#3}
\newcommand{\ltsel}[5]{\gpart{#1}\!\oplus\!\{#2: #3\}_{#4 \in #5}}
\newcommand{\ltbra}[5]{\gpart{#1}\&\{#2: #3\}_{#4 \in #5}}

%%%% NEW LOCAL TYOES, with cursor
\newcommand{\ltoutp}[3]{\gpart{#1}!\langle#2\rangle.\past #3}
\newcommand{\ltinpp}[3]{\gpart{#1}?\langle#2\rangle.\past #3}
\newcommand{\ltselp}[4]{\gpart{#1}\!\oplus\!\{#2\}_{#3 \in #4}}
\newcommand{\ltbrap}[4]{\gpart{#1}\&\{#2\}_{#3 \in #4}}



\newcommand{\tproj}[2]{#1\!\downarrow_{#2}}
\newcommand{\pproj}[3]{[\![#1]\!]^{#3}\downarrow_{#2}}

%stack based context%
%\newcommand{\conf}[2]{\Lbag #1 \; ; #2\; \Rbag}
\newcommand{\conf}[2]{\lbag #1 \; \textcolor{magenta}{\textbf{;}}\; #2 \rbag}
\newcommand{\stack}[1]{\mathtt{#1}}

%reductions%

\newcommand{\fwg}{\ensuremath{\fwcolor{\,\hookrightarrow\,}}}
\newcommand{\fwgs}{\ensuremath{\fwcolor{\,\hookrightarrow^*\,}}}
\newcommand{\bkg}{\ensuremath{\bkcolor{\,\rightharpoonup\,}}}
\newcommand{\bkgs}{\ensuremath{\bkcolor{\,\rightharpoonup^*\,}}}

\newcommand{\fw}{\ensuremath{\fwcolor{\,\twoheadrightarrow\,}}}
\newcommand{\fws}{\ensuremath{\fwcolor{\,\twoheadrightarrow^*\,}}}
\newcommand{\bk}{\ensuremath{\bkcolor{\,\rightsquigarrow\,}}}
\newcommand{\bks}{\ensuremath{\bkcolor{\,\rightsquigarrow^*\,}}}

\newcommand{\bkk}{\ensuremath{\bkcolor{\,\rightsquigarrow^{\,j}\,}}}
\newcommand{\trans}[1]{#1^{*}}
\newcommand{\refl}[1]{#1^{+}}
\newcommand{\fwa}{\ensuremath{\fwcolor{\Rrightarrow}}}
\newcommand{\lfwa}[1]{\xRightarrow{#1}}
\newcommand{\reda}{\rightarrowtail}
\newcommand{\lreda}[1]{\xRightarrow{#1}}

%equivalences%
%\newcommand{\bf}{\stackrel{\cdot}{\sim}}
%\newcommand{\bfw}{\stackrel{\cdot}{\approx}}
\newcommand{\bfb}{\sim}
\newcommand{\bfbw}{\approx}
\newcommand{\congruence}[1]{\stackrel{\cdot}{#1}}
\newcommand{\bka}{\ensuremath{\bkcolor{\Lleftarrow}}}
\newcommand{\lbka}{\xrightleftharpoons}

\newcommand{\ltrans}[1]{\xleftrightarrow{#1}}
%\newcommand{\simred}{\leftrightarrow}
\newcommand{\memstamp}{\eta}

\newcommand{\initC}[3]{\ensuremath{\mathcal{I}_{\,#3}^{#2}(#1)}}
\newcommand{\trad}[1]{\llbracket#1\rrbracket}

%stable conf%
\newcommand{\stable}{\mathtt{sb}}
\newcommand{\stables}[1]{#1\text{-}\stable}

\newcommand{\trace}{\rho}
\newcommand{\etrace}{\varepsilon}
\newcommand{\causeq}{\asymp}
\newcommand{\nottrace}[1]{{#1}_\bullet}
\newcommand{\tsource}[1]{\mathtt{src}(#1)}
\newcommand{\ttarget}[1]{\mathtt{trg}(#1)}

%%
\newcommand{\st}{\,|\,}
%jorge global macro%
\newcommand{\adeq}[2]{#1 \bowtie #2}
\newcommand{\ladeq}[3]{#1 \bowtie_{\,#3} #2}
\newcommand{\gth}[1]{\mathsf{#1}}
\newcommand{\ifk}{\mathbf{if}}
\newcommand{\thenk}{\mathbf{then}}
\newcommand{\elsek}{\mathbf{else}}
\newcommand{\ifproc}[3]{\ifk\,#1\, \thenk\, #2\,\elsek\,#3 }
\newcommand{\party}[1]{\ensuremath{\mathtt{#1}}\xspace}
\newcommand{\bigvect}[1]{\widehat{#1}}
\newcommand{\names}[1]{\mathtt{\mathbf{roles}}(#1)}



==> semdec.tex <==
% !TEX root = revchor.tex




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{figure*}[t!]
{%\small
\begin{mathpar}
\inferrule*[left=\fwcolor{(Init)}]
{\parties{G}= \{\p_1,\cdots,\p_n\} \and 
\forall \gpart{p}_i\in \parties{G}. \, \tproj{G}{\gpart{p}_i} = T_{i}  } 
{ 
\begin{array}{c}
\myloc{\loc_1}{\bout{a}{x_1:T_1}{P_{1}}} \Par 
\prod_{i \in \{2, \cdots, n\}}\myloc{\loc_i}{\binp{a}{x_i:T_i}{P_{i}}} 
\\
~\fw~ 
\\
\news{s} \Big(\, 
\prod_{i \in\{1,\cdots,n\}} \np{\key{\loc_i}{\p_i}}{ \conf{\inact}{P_i\subst{\ep{s}{\p_i}}{x_i}}} \Par 
\moni{s_{\p_i}}{\past T_{i}}{x_i}{\upd{x_i}{a }}  \Par \codah{s}{\emp}{\emp}{}\Big)
\end{array}
}
\and
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\inferrule*[left = \fwcolor{(Out)}]{ \p = \er \,\vee\, \p \in \names{\er, h_i} }{
\begin{array}{c}
\np{\key{\loc}{\er}}{ \conf{\stack{C}}{\bout{\ep{s}{\p}}{V}{P}}} \Par \moni{s_\p}{\myctxr{\ctx{T}}{\past  \ltout{\q}{U}{S}}}{\mytilde x}{\store} \Par \codah{s}{h_i}{h_o}{}  
\\
\fw 
\\
\np{\key{\loc}{\er}}{\conf{\stack{C}}{P}} \Par \moni{s_\p}{\myctxr{\ctx{T}}{ \ltoutp{\q}{U}{S}}}{\mytilde x}{\store} \Par 
\codah{s}{h_i}{h_o\cons \valueq{\p}{\q}{\myeval{V}{\sigma}}}{}
\end{array}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\and 
%
\inferrule*[left = \fwcolor{(In)}]{
\p = \er \,\vee\, \p \in \names{\er, h_i}
}
{\begin{array}{c}
\np{\key{\loc}{\er}}{\conf{\stack{C}}{\binp{\ep{s}{\p}}{y}{P}}} \Par \moni{s_\p}{\myctxr{\ctx{T}}{\past  \ltinp{\q}{U}{S}}}{\mytilde x}{\store} \Par \codah{s}{h_i}{\valueq{\q}{\p}{V}\cons h_o }{}
\\
\fw 
\\
\np{\key{\loc}{\er}}{\conf{\stack{C}}{P}} \Par \moni{s_\p}{ \myctxr{\ctx{T}}{\ltinpp{\q}{U}{S}}}{\mytilde x, y}{\store\upd{y}{V}} \Par 
\codah{s}{h_i\cons  \valueq{\q}{\p}{V}}{h_o }{} 
\end{array}
} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\and
\inferrule[\fwcolor{(Sel)}]
{\p = \er \,\vee\, \p \in \names{\er, h_i}
\and
w\in J \and J\subseteq I }
{ 
\begin{array}{c}
\np{\key{\loc}{\er}}{ \conf{\stack C}{\bsel{\ep{s}{\p}}{\lbl_i. P_i}_{i\in I}}}  \Par 
\moni{s_\p}{\myctxr{\ctx{T}}{\past \ltsel{\q}{\lbl_j}{S_j}{j}{J}} }{\mytilde x}{\store} \Par \codah{s}{h_i}{h_o}{} \quad 
\\
\fw 
\\
\np{\key{\loc}{\er}}{ \conf{\stack C , \bsel{\ep{s}{\p}}{\lbl_i.P_i}_{i\in I\setminus w} }{P_w} }\Par 
\moni{s_\p}{ \myctxr{\ctx{T}}{ \ltselp{\q}{\lbl_j:S_j \, , \, \lbl_w:\past S_w}{j}{J\setminus w}} }{\mytilde x}{\store} 
%\\
%\quad \qquad
\Par 
\codah{s}{h_i}{h_o\cons  \valueq{\p}{\q}{\lbl_w} }{} 
\end{array} 
 }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\and
\inferrule[\fwcolor{(Bra)}]{\p = \er \,\vee\, \p \in \names{\er, h_i} 
\and w\in I \and I\subseteq J }
{
\begin{array}{c}
\np{\key{\loc}{\er}}{ \conf { \stack C}{\bbra{\ep{s}{\p}}{\lbl_i:P_i}_{i \in I} } } \Par \moni{s_\p}{\myctxr{\ctx{T}}
{\past \ltbra{\q}{\lbl_j}{S_j}{j}{J}} }{\mytilde x}{\store} \Par \codah{s}{h_i}{\valueq{\q}{\p}{\lbl_w}\cons h_o}{} 
\\
\fw 
\\
\np{\key{\loc}{\er}}{ \conf { \stack C , \bbra{\ep{s}{\p}}{\lbl_i:P_i}_{i \in I\setminus w}}{ P_w} } \Par 
\moni{s_\p}{\myctxr{\ctx{T}}{\ltbrap{\q}{\lbl_j:S_j\,,\, \lbl_w:\past S_w}{j}{J\setminus w}} }{\mytilde x}{\store}
%\\
%\quad  \qquad 
\Par \codah{s}{h_i\cons  \valueq{\q}{\p}{\lbl_w}}{h_o}{}
\end{array}
 }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\and
%
\inferrule[\fwcolor{(Beta)}]{\myeval{V}{\sigma} =\abs{x}{P} }
{
\begin{array}{l}
\np{\key{\loc}{\p}}{\conf{\stack{C}}{(\appl{V}{w})}} \Par \moni{s_\p}{\myctxr{\ctx{T}}{\past S}}{\mytilde x}{\store} 
~\fw~ 
\news{k}\, \left( {\np{\key{\loc}{\p}}{\conf{\ctx{\stack {C}}}{P\subst{\myeval{w}{\sigma}}{x}}}}  \Par \mem{k}{(\appl{V}{w})}{\loc} \Par\moni{s_\p}{\myctxr{\ctx T}{ k. \past S}}{\mytilde x}{\store} \right)
\end{array}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\and
%
\inferrule[\fwcolor{(Spawn)}]{ }
{
\begin{array}{c}
\np{\key{\loc}{\p}}{\conf{\stack{C}}{P \Par Q}} \Par \moni{s_\p}{\myctxr{\ctx{T}}{\past S}}{\mytilde x}{\store} 
\\
~\fw~ 
\\
\news{\loc_1,\loc_2}\, \left( \np{\key{\loc}{\p}}{\conf{\stack{C}}{\inact}}  
\Par \np{\key{\loc_1}{\p}}{\conf{\inact}{P}}
\Par \np{\key{\loc_2}{\p}}{\conf{\inact}{Q}} 
\Par \moni{s_\p}{\myctxr{\ctx T}{ (\loc,\loc_1,\loc_2). \past S}}{\mytilde x}{\store} \right)
\end{array}
}

\end{mathpar}
}
\vspace{-5mm}
\caption{Decoupled semantics for configurations: Forward reduction ($\fw$).}
\label{fig:fw}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[t!]
{%\small
\begin{mathpar}
\inferrule*[left=\bkcolor{(RInit)}]
{\parties{G}= \{\p_1,\cdots,\p_n\} \and 
\forall \gpart{p}_i\in \parties{G}. \, \tproj{G}{\gpart{p}_i} = T_{i} \and P_i = Q_{i}\subst{\ep{s}{\p_i}}{x} } 
{ 
\begin{array}{c}
\news{s} \left(\, 
\prod_{i \in\{1,\cdots,n\}} \np{\key{\loc_i}{\p_i}}{ \conf{\inact}{Q_i}} \Par 
\hmoni{s_{\p_i}}{\past T_{i}}{x_i}{\upd{x_i}{a }}  \Par \codah{s}{\emp}{\emp}{}\right)
\\
~\bk~
\\
\myloc{\loc_1}{\bout{a}{x_1:T_1}{P_{1}}} \Par 
\prod_{i \in \{2, \cdots, n\}} \myloc{\loc_i}{\binp{a}{x_i:T_i}{P_i}}
\end{array}
}
\and
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\inferrule*[left=\bkcolor{(RollS)}]{ }{
\begin{array}{c}
\hmoni{s_\p}{ \myctxr{\ctx T}{\ltinpp{\q}{U}{T}}}{\mytilde x}{\store_1} \Par 
\hmoni{s_\q}{ \myctxr{\ctx S}{\ltoutp{\p}{U}{S}}}{\mytilde y}{\store_2} \Par 
%\codah{s}{h_i}{h_o}{\restrict{\mytilde{\gpart{r}}}}
\codah{s}{h_i}{h_o}
%\quad 
\\
\bk 
\\
\monir{s_\p}{ \myctxr{\ctx T}{\ltinpp{\q}{U}{T}}}{\mytilde x}{\store_1} \Par 
\monir{s_\q}{\myctxr{\ctx S}{\ltoutp{\p}{U}{S}}}{\mytilde y}{\store_2} \Par 
%\codah{s}{h_i}{h_o}{\restrict{\mytilde{\gpart{r}},\p,\q}}
\codah{s}{h_i}{h_o}
\end{array}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\and 
%
\inferrule[\bkcolor{(RollC)}]{ }{
\begin{array}{c}
\hmoni{s_\p}{\myctxr{\ctx T}{\ltbrap{\q}{\lbl_z:\past S_z\,,\,\lbl_w:S_w}{z}{J\setminus w}}}{\mytilde x}{\store_1}  \Par 
\hmoni{s_\q}{\myctxr{\ctx S}{\ltselp{\p}{\lbl_z:\past S_z \, , \, \lbl_w: S_w}{z}{J\setminus w}}}{\mytilde y}{\store_2}  \Par 
%\codah{s}{h_i}{h_o}{\restrict{\mytilde{\gpart{r}}}}
\codah{s}{h_i}{h_o}
\\
\bk 
\\
\monir{s_\p}{ \myctxr{\ctx T}{\ltbrap{\q}{\lbl_z:\past S_z\,,\,\lbl_w:S_w}{z}{J\setminus w}}}{\mytilde x}{\store_1}  \Par 
\monir{s_\q}{\myctxr{\ctx S}{\ltselp{\p}{\lbl_z:\past S_z \, , \, \lbl_w: S_w}{z}{J\setminus w}}}{\mytilde y}{\store_2}  \Par 
%\codah{s}{h_1}{h_2}{\restrict{\mytilde{\gpart{r}},\p,\q}}
\codah{s}{h_i}{h_o}
\end{array}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\and
%
\inferrule*[left=\bkcolor{(ROut)}]{ \p = \er \,\vee\, \p \in \names{\er, h_i}}
{
\begin{array}{l}
\np{\key{\loc}{\er}}{\conf{\stack C}{P}} \Par \monir{s_\p}{ \myctxr{\ctx T}{\ltoutp{\q}{U}{S}} }{\mytilde x}{\store}
\Par 
%\codah{s}{h_i}{(\p,\q,V)\cons h_o}{\restrict{\p,\mytilde{\gpart{r}}}}
\codah{s}{h_i}{(\p,\q,V)\cons h_o}
\\
~\bk~
\\
\np{\key{\loc}{\er}}{\conf{\stack C }{\bout{\ep{s}{\p}}{V}{P}}} \Par 
\hmoni{s_\p}{ \myctxr{\ctx T}{\past\ltout{\q}{U}{S}} }{\mytilde x}{\store}
 \Par %\codah{s}{h_i}{h_o}{\restrict{\mytilde{\gpart{r}}}}
 \codah{s}{h_i}{h_o}
\end{array}
 }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\and
%
\inferrule*[left=\bkcolor{(RIn)}]{ 
\p = \er \,\vee\, \p \in \names{\er, h_i}
}
{
\begin{array}{c}
\np{\key{\loc}{\er}}{\conf{\stack C}{P}} \Par 
\monir{s_\p}{ \myctxr{\ctx T} {\ltinpp{\q}{U}{S}} }{\mytilde x,y}{\store} \Par 
%\codah{s}{h_i\cons(\q,\p,V)}{h_o}{\restrict{\p,\mytilde{\gpart{r}}}}
\codah{s}{h_i\cons(\q,\p,V)}{h_o}
\\
\quad \bk
\\
\np{\key{\loc}{\er}}{\conf{\stack C} { \binp{\ep{s}{\p}}{y}{P}} } \Par 
\hmoni{s_\p}{ \myctxr{\ctx T}{\past\ltinp{\q}{U}{S}}}{\mytilde x}{\rup{\store}{y}}\Par %\codah{s}{h_i}{(\q,\p,V)\cons h_o}{\restrict{\mytilde{\gpart{r}}}}
\codah{s}{h_i}{(\q,\p,V)\cons h_o}
\end{array}
 }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\and
\inferrule[\bkcolor{(RBra)}]
{ \p = \er \,\vee\, \p \in \names{\er, h_i} \and w \in I \and I\subseteq J} 
{
\begin{array}{c}
\np{\key{\loc}{\er}}{\conf{\stack C,\bbra{\ep{s}{\p}}{\lbl_i:P_i }_{i \in I\setminus\set{w}}}{P}
} \Par 
\monir{s_\p}{\myctxr{\ctx T}{\ltbrap{\q}{\lbl_j:S_j\,,\, \lbl_w:\past S_w}{j}{J\setminus w}} }{\mytilde x}{\store}
\Par 
%\codah{s}{h_i\cons  \valueq{\q}{\p}{\lbl_w}}{h_o}{\restrict{\p, \mytilde{\gpart{r}}}}
\codah{s}{h_i\cons  \valueq{\q}{\p}{\lbl_w}}{h_o}
\\
\quad \bk 
\\%[1mm]
\np{\key{\loc}{\er}}{ \conf{\stack C}{\bbra{\ep{s}{\p}}{\lbl_i:P_i, \lbl_w : P }_{i \in I\setminus\set{w}}}} \Par 
\hmoni{s_\p}{\myctxr{\ctx T}{\past\ltbra{\q}{\lbl_j}{S_j}{j}{J}} }{\mytilde x}{\store} 
\Par 
%\codah{s}{h_i}{\valueq{\q}{\p}{\lbl_w}\cons h_o}{\restrict{\mytilde{\gpart{r}}}}
\codah{s}{h_i}{\valueq{\q}{\p}{\lbl_w}\cons h_o}
\end{array}
 }
\and 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\inferrule*[left=\bkcolor{(RSel)}]
{ \p = \er \,\vee\, \p \in \names{\er, h_i} \and w \in I \and I\subseteq J} 
{
\begin{array}{c}
\np{{\key{\loc}{\er}}}{ \conf{\stack C,\bsel{\ep{s}{\p}}{\lbl_i. P_i}_{i\in I} }{P}} \Par 
\monir{s_\p}{ \myctxr{\ctx T}{ \ltselp{\q}{\lbl_j:S_j \, , \, \lbl_w:\past S_w}{j}{J\setminus w} } }{\mytilde x}{\store}
\Par 
%\codah{s}{h_i}{\valueq{\p}{\q}{\lbl_w}\cons h_o}{\restrict{\p,\mytilde{\gpart{r}}}}
\codah{s}{h_i}{\valueq{\p}{\q}{\lbl_w}\cons h_o}
\\
\quad \bk 
\\
\np{{\key{\loc}{\er}}}{ \conf{\stack C}{ \bsel{\ep{s}{\p}}{\lbl_w. P} + \bsel{\ep{s}{\p}}{\lbl_i. P_i}_{i\in I} } } \Par 
\hmoni{s_\p}{ \myctxr{\ctx T}{ \past \ltsel{\q}{\lbl_j}{S_j}{j}{J} } }{\mytilde x}{\store} \Par 
%\codah{s}{h_i}{h_o}{\restrict{\mytilde{\gpart{r}}}}
\codah{s}{h_i}{h_o}
\end{array}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\and
%
\inferrule*[left=\bkcolor{(RBeta)}]{ }
{
\begin{array}{l}
\news{k}\,\left( {\np{\key{\loc}{\p}}{\conf{\stack{C}}{Q} }}  \Par \mem{k}{(\appl{V}{w})}{\loc} \Par\moni{s_\p}{\myctxr{\ctx T}{ k. \past S}}{\mytilde x}{\store}
\right)
%\\
~\bk~ 
%\\
\np{\key{\loc}{\p}}{\conf{\stack{C}}{(\appl{V}{w})}} \Par \moni{s_\p}{\myctxr{\ctx{T}}{\past S}}{\mytilde x}{\store} 
\end{array} 
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \and
\inferrule[\bkcolor{(RSpawn)}]{ }
{
\begin{array}{c}
\news{\loc_1,\loc_2}\, \left( {\np{\key{\loc}{\p}}{\conf{\stack{C}}{\inact}}}  
\Par \np{\key{\loc_1}{\p}}{\conf{\inact}{P}}
\Par \np{\key{\loc_2}{\p}}{\conf{\inact}{Q}} 
\Par \moni{s_\p}{\myctxr{\ctx T}{ (\loc,\loc_1,\loc_2). \past S}}{\mytilde x}{\store} \right)
\\
~\bk~
\\
\np{\key{\loc}{\p}}{\conf{\stack{C}}{P \Par Q}} \Par \moni{s_\p}{\myctxr{\ctx{T}}{\past S}}{\mytilde x}{\store}  
\end{array}
}

\end{mathpar}
}
\vspace{-4mm}
\caption{Decoupled semantics for configurations: Backwards reduction ($\bk$).}
\label{fig:bk}
\vspace{-3mm}
\end{figure*}

